Streaming Algorithms for Ellipsoidal Approximation of Convex Polytopes

We give efficient deterministic one-pass streaming algorithms for finding an ellipsoidal approximation of a symmetric convex polytope. The algorithms are near-optimal in that their approximation factors differ from that of the optimal offline solution only by a factor sub-logarithmic in the aspect ratio of the polytope.

==> includes_arxiv.tex <==
\usepackage{amsmath,amssymb,amsthm}
\usepackage{amsmath}[fleqn]
\usepackage{amsthm,amssymb}
\usepackage{xcolor}
\usepackage{mathtools}
\usepackage{enumitem}
\usepackage{bbm}
\usepackage{semantic}
\usepackage{listings}
\usepackage{courier}
\usepackage{tikz}
\usetikzlibrary{calc}
\usepackage{color}
\usepackage{fancyhdr}
\usepackage{lastpage}
% \usepackage{subcaption}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}
 
\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2,
    basicstyle=\footnotesize\ttfamily
}

\lstset{style=mystyle}

\usepackage[colorlinks = true,
            linkcolor = blue,
            urlcolor  = blue,
            citecolor = blue,
            anchorcolor = blue]{hyperref}

% \DeclareMathOperator*{\E}{\mathbb{E}}
\let\Pr\relax
\DeclareMathOperator*{\Pr}{\mathrm{Pr}}

\newcommand{\eps}{\epsilon}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\inprod}[1]{\left\langle #1 \right\rangle}
% \newcommand{\R}{\mathbb{R}}
\renewcommand{\S}{\mathbb{S}}

% \newcommand{\norm}[1]{\left\lVert#1\right\rVert}
% \newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\paren}[1]{\left(#1\right)}
\newcommand{\innerprod}[1]{\left\langle#1\right\rangle}
\newcommand{\sqb}[1]{\left[#1\right]}
\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}
\newcommand{\setmath}[1]{\left\{#1\right\}}
\newcommand*\xor{\mathbin{\oplus}}
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor}
\newcommand{\bigoh}[1]{\mathcal{O}\paren{#1}}
\newcommand{\gaussian}[2]{\mathcal{N}\paren{#1, #2}}
\newcommand{\myfunc}[3]{#1\colon#2\to#3}
\newcommand{\Unif}[1]{\mathsf{Unif}\inparen{#1}}
\newcommand{\otilde}[1]{\widetilde{O}\inparen{#1}}

% \usepackage{fancybox}
% \makeatletter
% \newtheoremstyle{caja}
%   {\topsep}
%   {\topsep}
%   {\itshape}
%   {}
%   {\bfseries}
%   {}
%   {.5em}
%   {\ovalbox{\thmname{#1}~\thmnumber{#2}\@ifempty{#3}{.}{}\thmnote{ (#3).}}}
% \makeatother

% \theoremstyle{caja}
% \theoremstyle{definition}

\newenvironment{proofoutline}
 {\renewcommand\qedsymbol{}\proof[Proof outline]}
 {\endproof}

% \newtheorem{theorem}{Theorem}[section]
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{remark}{Remark}
\newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{lemma}{Lemma}[section]
\newtheorem{example}[theorem]{Example}
% \newtheorem{example}{Example}[section]
\newtheorem{observation}[theorem]{Observation}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
% \newtheorem{definition}{Definition}[section]
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
% \newtheorem{fact}{Fact}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{problem}[theorem]{Problem}
\newtheorem{question}{Question}
% \newtheorem{problem}{Problem}
\newtheorem{exercise}{Exercise}
\numberwithin{exercise}{section}
% \numberwithin{problem}{subsection}
\newenvironment{solution}
  {\begin{proof}[Solution]}
  {\end{proof}}

\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand*\Diff[1]{\mathop{}\!\mathrm{d^#1}}

\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\prox}{prox}
% \DeclareMathOperator{\var}{var}
\DeclareMathOperator{\dom}{dom}
% \DeclareMathOperator{\rk}{rk}
\DeclareMathOperator{\nul}{nul}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\dual}{dual}
\DeclareMathOperator{\im}{im}
% \DeclareMathOperator{\Span}{Span}
\newcommand{\Span}{\mathsf{Span}}
\DeclareMathOperator{\cost}{cost}

\newcommand{\exv}[1]{\E\sqb{#1}}
\newcommand{\exvv}[2]{\underset{#1}{\E}\sqb{#2}}
\newcommand{\expv}[1]{\mathsf{exp}\paren{#1}}
\newcommand{\prv}[1]{\Pr\sqb{#1}}
\newcommand{\prvv}[2]{\underset{#1}{\Pr}\sqb{#2}}
\newcommand{\logv}[1]{\log\paren{#1}}
\newcommand{\diag}[1]{\mathsf{diag}\paren{#1}}
\newcommand{\diam}[1]{\mathsf{diam}\paren{#1}}
\newcommand{\linf}{\ell_{\infty}}
\newcommand{\costv}[1]{\cost\paren{#1}}
\newcommand{\err}[2]{\mathsf{err}_{#1}\inparen{#2}}
\newcommand{\signv}[1]{\sign\inparen{#1}}
\newcommand{\trv}[1]{\Tr\inparen{#1}}
% \newcommand{\suchthat}{~\middle|~}

\renewcommand{\vec}[1]{\overrightarrow{#1}}

\makeatletter
\newcommand{\vo}{\vec{o}\@ifnextchar{^}{\,}{}}
\makeatother

\newcommand*{\vertbar}{\rule[-1ex]{0.5pt}{2.5ex}}
\newcommand*{\horzbar}{\rule[.5ex]{2.5ex}{0.5pt}}

\newcommand{\mvar}[1]{\mathit{#1}}
\newcommand{\qt}[1]{\mbox{`#1'}}

\usepackage{tcolorbox}
% \usepackage{subfigure} 

% For citations
% \usepackage{natbib}

% For algorithms
\usepackage{algorithm}
\usepackage{algorithmic}

% disable the below lines if you want auto-indent
\newlength\tindent
\setlength{\tindent}{\parindent}
\setlength{\parindent}{0pt}
\renewcommand{\indent}{\hspace*{\tindent}}

\numberwithin{equation}{section}

%%%%%%%%%% Symbols and Fonts
\def\from{:}
\def\to{\rightarrow}
\def\eps{\varepsilon}
\def\epsilon{\varepsilon}
\def\e{\epsilon}
\def\eps{\epsilon}
\def\d{\delta}
\def\phi{\varphi}
\def\cal{\mathcal}
\def\xor{\oplus}
\def\ra{\rightarrow}
\def\implies{\Rightarrow}
\def\psdgeq{\succeq} 
\renewcommand{\bar}{\overline} 
\newcommand{\ol}{\overline}

\def\bull{\vrule height .9ex width .8ex depth -.1ex }

%%%%%%%%%%%%%%%%%%%%%% Text Macros
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\etal}{et al.\xspace}
\newcommand{\cf}{{\it cf.,}}

%%%%%%%%%%%%%%%%%%%%% Punctuation at the end of a displayed formula
\newcommand{\mper}{\,.}
\newcommand{\mcom}{\,,}

%%%%%%%%%%%%%%%%%%%%%% Number Sets
\newcommand{\R}{{\mathbb R}}
\newcommand{\E}{{\mathbb E}}
\newcommand{\C}{{\mathbb C}}
\newcommand{\Q}{{\mathbb Q}}
\newcommand{\N}{{\mathbb{N}}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\F}{{\mathbb F}}
\newcommand{\T}{{\mathbb T}}
\newcommand{\zo}{\{0,1\}}
\newcommand{\GF}{\mathrm{GF}}
\newcommand{\FF}{{\mathbb F}}
\newcommand{\Real}{{\mathbb R}}

\newcommand{\indicator}[1]{\mathbbm{1}\inbraces{#1}}

%%%%%%%%%%%%%%%%%%%%% Random Variables and Probability
\newcommand{\Esymb}{\mathbb{E}}
\newcommand{\Psymb}{\mathbb{P}}
\newcommand{\Vsymb}{\mathsf{Var}}

\DeclareMathOperator*{\ExpOp}{\Esymb}
\DeclareMathOperator*{\VarOp}{\Vsymb}
% \DeclareMathOperator*{\ProbOp}{\Psymb}
% \renewcommand{\Pr}{\ProbOp}
\renewcommand{\Pr}{\mathsf{Pr}}

\newcommand{\prob}[1]{\Pr\left[{#1}\right]}
\newcommand{\Prob}[2]{\Pr_{{#1}}\left[{#2}\right]}
\newcommand{\ex}[1]{\ExpOp\left[{#1}\right]}
\newcommand{\Ex}[2]{\ExpOp_{{#1}}\left[{#2}\right]}
\newcommand{\var}[1]{\VarOp\left[{#1}\right]}
\newcommand{\Var}[2]{\VarOp_{{#1}}\left[{#2}\right]}
\newcommand{\covar}[1]{\mathsf{Cov}\insquare{#1}}
\newcommand{\stablerank}[1]{\mathsf{sr}\inparen{#1}}
\newcommand{\rank}[1]{\mathsf{rk}\inparen{#1}}

% \newcommand{\comp}{\mathsf{c}}


\newcommand{\conv}[1]{\mathsf{conv}\inparen{#1}}
\newcommand{\given}{\;\middle\vert\;}


%%%%%%%%%% Standard Normal Distribution
\newcommand{\gauss}[2]{{\cal N(#1, #2)}}

%%%%%%%%%%%% Fractions
% commands for fractions 
\usepackage{nicefrac}
% poor man's fraction
\newcommand{\flatfrac}[2]{#1/#2}
\newcommand{\varflatfrac}[2]{#1\textfractionsolidus#2}

\let\nfrac=\nicefrac
\let\ffrac=\flatfrac
% similar commands: tfrac,dfrac

\newcommand{\half}{\nicefrac12}
\newcommand{\onequarter}{\nicefrac14}
\newcommand{\threequarter}{\nicefrac34}

%%%%%%%%%%%%%%%%%% Vectors and Reals
\newcommand{\abs}[1]{\ensuremath{\left\lvert #1 \right\rvert}}
\newcommand{\smallabs}[1]{\ensuremath{\lvert #1 \rvert}}
%
\newcommand{\norm}[1]{\ensuremath{\left\lVert #1 \right\rVert}}
\newcommand{\opnorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{\mathrm{op}}}}
\newcommand{\maxnorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{\infty}}}
\newcommand{\fnorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{F}}}
\newcommand{\lipnorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{\mathrm{Lip}}}}
\newcommand{\onenorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{1}}}
\newcommand{\zeronorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{0}}}
\newcommand{\nuclearnorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{*}}}
\newcommand{\smallnorm}[1]{\ensuremath{\lVert #1 \rVert}}
%
\newcommand{\mydot}[2]{\ensuremath{\left\langle #1, #2 \right\rangle}}
\newcommand{\mysmalldot}[2]{\ensuremath{\langle #1, #2 \rangle}}
\newcommand{\ip}[1]{\left\langle #1 \right\rangle}

%%%%%%%%%%% Vectors
\def\bfx {{\bf x}}
\def\bfy {{\bf y}}
\def\bfz {{\bf z}}
\def\bfu{{\bf u}}
\def\bfv{{\bf v}}
\def\bfw{{\bf w}}
\def\bfa{{\bf a}}
\def\bfb{{\bf b}}
\def\bfc{{\bf c}}
\def\bfg{{\bf g}}

\newcommand{\zero}{\mathbf 0}
\newcommand{\one}{{\mathbf{1}}}
\newcommand{\zeroone}{{0/1}\xspace}
\newcommand{\minusoneone}{{-1/1}\xspace}

\newcommand{\yes}{{\sf Yes}\xspace}
\newcommand{\no}{{\sf No}\xspace}


%%%%%%%%%%%%%%%%%%%%%% General Useful Macros
\newfont{\inhead}{eufm10 scaled\magstep1}
\newcommand{\deffont}{\sf}

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{C}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\poly}{{\mathrm{poly}}}
\newcommand{\polylog}{{\mathrm{polylog}}}
\newcommand{\loglog}{{\mathop{\mathrm{loglog}}}}
\newcommand{\suchthat}{{\;\; : \;\;}}
\newcommand{\getsr}{\mathbin{\stackrel{\mbox{\tiny R}}{\gets}}}


%%%%%%%%%% Operators
\DeclareMathOperator\supp{Supp}
\newcommand{\argmax}{\mathrm{argmax}}
\newcommand{\argmin}{\mathrm{argmin}}
\newcommand{\suppv}[1]{\mathsf{Supp}\inparen{#1}}

%%%%%%%%%%%%%%%%%%% Complexity Classes
\newcommand{\classfont}[1]{\textsf{#1}}
\newcommand{\coclass}[1]{\mathbf{co\mbox{-}#1}} 
\newcommand{\BPP}{\classfont{BPP}\xspace}
\newcommand{\classP}{\classfont{P}\xspace}
\newcommand{\NP}{\classfont{NP}\xspace}
\newcommand{\coNP}{\classfont{coNP}\xspace}
\newcommand{\nphard}{\classfont{NP}-hard\xspace}

%%%%%%%%%%%%%%%%%%%% Problems
% use texorpdfstring to avoid problems with hyperref (can use problem
% macros also in headings
\newcommand{\problemmacro}[1]{\textsf{#1}}

\newcommand{\maxcsp}{\problemmacro{MAX-CSP}\xspace}
\newcommand{\maxkcsp}{\problemmacro{MAX k-CSP}\xspace}
\newcommand{\maxthreesat}{\problemmacro{MAX 3-SAT}\xspace}
\newcommand{\maxthreexor}{\problemmacro{MAX 3-XOR}\xspace}
\newcommand{\maxkxor}{\problemmacro{MAX k-XOR}\xspace}
\newcommand{\maxcut}{\problemmacro{MAX-CUT}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%% Enclosures
\newcommand{\inparen}[1]{\left(#1\right)}             %\inparen{x+y}  is (x+y)
\newcommand{\inbraces}[1]{\left\{#1\right\}}           %\inbrace{x+y}  is {x+y}
\newcommand{\insquare}[1]{\left[#1\right]}             %\insquare{x+y}  is [x+y]
\newcommand{\inangle}[1]{\left\langle#1\right\rangle} %\inangle{A}    is <A>
\newcommand{\inmod}[1]{\inparen{\mathrm{mod}\ #1}}

\newcommand{\B}{\inbraces{0,1}}
\newcommand{\pmone}{\inbraces{\pm1}}


%%%%%%%%%%%%%%%%%%%% Names
\newcommand{\Erdos}{Erd\H{o}s\xspace}
\newcommand{\Renyi}{R\'enyi\xspace}
\newcommand{\Lovasz}{Lov\'asz\xspace}
\newcommand{\Juhasz}{Juh\'asz\xspace}
\newcommand{\Bollobas}{Bollob\'as\xspace}
\newcommand{\Furedi}{F\"uredi\xspace}
\newcommand{\Komlos}{Koml\'os\xspace}
\newcommand{\Luczak}{\L uczak\xspace}
\newcommand{\Kucera}{Ku\v{c}era\xspace}
\newcommand{\Szemeredi}{Szemer\'edi\xspace}
\newcommand{\Chvatal}{Chv\'atal}
\newcommand{\Holder}{H\"{o}lder}
\newcommand{\Plunnecke}{Pl\"unnecke}

%%%%%%%%%% Symbols and Fonts
\def\from{:}
\def\to{\rightarrow}
\def\eps{\varepsilon}
\def\epsilon{\varepsilon}
\def\e{\epsilon}
\def\eps{\epsilon}
\def\d{\delta}
\def\phi{\varphi}
\def\cal{\mathcal}
\def\xor{\oplus}
\def\ra{\rightarrow}
\def\implies{\Rightarrow}
\def\psdgeq{\succeq} 
\renewcommand{\bar}{\overline} 

\newcommand{\onev}{\mathbbm{1}}
\newcommand{\booland}{\wedge}
\newcommand{\boolor}{\vee}
\newcommand{\boolbigand}{\bigwedge}
\newcommand{\boolbigor}{\bigvee}

\newcommand{\vspan}[1]{\mathsf{Span}\inparen{#1}}
\newcommand{\defn}[1]{{\deffont {#1}}}
\newcommand{\phileft}{\phi_{\mathrm{left}}}
\newcommand{\kernel}[1]{\mathsf{Ker}\inparen{#1}}
\newcommand{\image}{\mathsf{im}}
\newcommand{\vdim}[1]{\mathsf{dim}\inparen{#1}}
\newcommand{\vrank}[1]{\mathsf{rank}\inparen{#1}}
\newcommand{\vc}[1]{\mathsf{VC}\inparen{#1}}
\newcommand{\covc}[1]{\mathsf{coVC}\inparen{#1}}
\newcommand{\id}{\mathsf{id}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\Xgood}{X_{\mathsf{good}}}
\newcommand{\Xbad}{X_{\mathsf{bad}}}
\newcommand{\Xhat}{\widehat{X}}
\newcommand{\hhat}{\widehat{h}}
\newcommand{\hstar}{h^{*}}
\newcommand{\Vhat}{\widehat{V}}
\newcommand{\Sigmahat}{\widehat{\Sigma}}

\newcommand{\pinv}[1]{#1^{+}}
\newcommand{\ppinv}[1]{\inparen{#1}^{+}}

\usepackage{multirow}
\usepackage{soul}

\usepackage{thmtools}
\usepackage{thm-restate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> main_alg_and_analysis_OLD.tex <==
\section{Revised Algorithm}
\label{section:revised_algorithm}

We now generalize Algorithm \ref{alg:greedy_maxev} to the case where we are instead given an approximation to the aspect ratio $\kappa(X)$. The advantage of this relaxed assumption is that we no longer have to make a data-dependent initialization. We give this revision in Algorithm \ref{alg:general_greedy_maxev}.

\begin{algorithm}[ht]
\caption{Streaming Ellipsoidal Approximation\label{alg:general_greedy_maxev}}
\begin{algorithmic}[1]
    \STATE \textbf{Input}: A stream from which to read $x_1, \dots, x_n$, and $K = q \cdot \kappa(X)$, a factor-$q \ge 1$ estimate of $\kappa(X)$.
    \STATE \textbf{Output}: Linear transformation $A_n$ satisfying $\cE_n = \inbraces{x \suchthat \norm{A_nx} \le 1}$, where $X = \conv{\inbraces{\pm x_1,\dots,\pm x_n}} \subseteq \cE_n$.
    \STATE Receive point $x_1$.
    \STATE Let $V_1^T$ be an orthogonal matrix satisfying $V_1^Tx_1 = e_1 \cdot \norm{x_1}$.
    \STATE Let $U_1 = I$.
    \STATE Let $\Sigma_1$ be $\diag{\nfrac{1}{\norm{x_1}}, \nfrac{K}{\norm{x_1}}, \dots, \nfrac{K}{\norm{x_1}}}$.
    \FOR{$t = 2, \ldots, n$}
        \STATE Receive point $x_t$.
        \IF{$\norm{\Sigma_{t-1}V_{t-1}^Tx_t} > 1$}
            \STATE Let $a \coloneqq \nfrac{U_{t-1}\Sigma_{t-1}V_{t-1}^Tx_t}{\norm{\Sigma_{t-1}V_{t-1}^Tx_t}}$.
            \STATE Let $b^T \coloneqq a^T(U_{t-1}\Sigma_{t-1}V_{t-1}^T)$.
            \STATE Let $U_t, \Sigma_t', V_t^T$ be such that $U_t\Sigma_t'V_t^T = U_{t-1}\Sigma_{t-1}V_{t-1}^T - \inparen{1 - \nfrac{1}{\norm{\Sigma_{t-1}V_{t-1}^Tx_t}}}ab^T$, where $U_t$ and $V_t^T$ are orthonormal matrices in $\R^{d\times d}$ and $\Sigma_t'$ is a diagonal matrix.\label{line:svd_update}
            \STATE Let $M_t \coloneqq \max_{1\leq i \leq t} \|x_i\|$.
            \STATE Denote the diagonal entries of $\Sigma_t'$ by $\Sigma_{1,t}', \dots, \Sigma_{i,d}'$. Let $\Sigma_{i,t} = \min\inbraces{\Sigma_{i,t}', \nfrac{K}{M_t}}$ for every $i \in [d]$.
            \STATE Let $\Sigma_t = \diag{\sigma_{1,t}, \dots, \sigma_{d,t}}$. \label{line:sv_correction}
        \ELSE
            \STATE $U_t = U_{t-1}$, $V_t^T = V_{t-1}^T, \Sigma_t = \Sigma_{t-1}$.
        \ENDIF
    \ENDFOR
    \STATE \textbf{Output}: $\cE_n = \inbraces{x \suchthat \norm{\Sigma_nV_n^Tx}\le 1}$.
\end{algorithmic}
\end{algorithm}

Observe the effect of Line \ref{line:sv_correction} is to correct the singular values of $A_t$ in order to keep it well-conditioned. We will refer to this this process as the ``singular value correction step.''

The remainder of this section is devoted to proving Theorem \ref{thm:greedy_approx}.\ynote{I would just assume that we are given $K\geq \kappa(X)$; that is, $q\geq 1$ and get rid of $q$.} \textcolor{red}{visualized implication chain?}

\mybox{\begin{theorem}
\label{thm:greedy_approx}
Suppose that we give Algorithm \ref{alg:general_greedy_maxev} a value of $K$ satisfying $K = q\cdot\kappa(X)$. Then, Algorithm \ref{alg:general_greedy_maxev} outputs an ellipsoid $\cE_n$ satisfying:
\begin{align*}
    \frac{\cE_n}{\sqrt{\magicnumber{\inparen{q\cdot\kappa(X)}}} \cdot \sqrt{1 + \nfrac{1}{q^2}}} \subseteq X \subseteq \cE_n
\end{align*}
In this sense, Algorithm \ref{alg:general_greedy_maxev} produces a $\sqrt{\magicnumber{\inparen{q\cdot\kappa(X)}}} \cdot \sqrt{1 + \nfrac{1}{q^2}}$-outer ellipsoidal approximation to $X$. Moreover, Algorithm \ref{alg:general_greedy_maxev} runs in time $O(nd^2\log^2d)$ and stores at most $O(d^2)$ floats.
\end{theorem}}
\begin{proof}
We first address performance concerns; then, we analyze the correctness.

\paragraph{Runtime and Memory Complexity}
It is easy to see that Algorithm \ref{alg:general_greedy_maxev} keeps track of three matrices $U_t, \Sigma_t, V_t^T$ at every iteration, in addition to the new point $x_t$. Algorithm \ref{alg:general_greedy_maxev} does not store anything else in between iterations, so the memory complexity is $O(d^2)$ floating-point numbers, as desired.

We now analyze the runtime. Observe that for all $w\in\R^d$, we have $U_{t-1}\Sigma_{t-1}V_{t-1}^Tw$ can be computed in time $O(d^2)$, as this product can be rewritten as three matrix-vector products. It now remains to show that we can implement Line \ref{line:svd_update} efficiently; this can be implemented in time $O(d^2\log^2 d)$ as per \cite{stange08}. Hence, each iteration takes time $O(d^2\log^2d)$ time, from which we have that Algorithm \ref{alg:general_greedy_maxev} has time complexity $O(nd^2\log^2d) = \widetilde{O}\inparen{nd^2}$, as desired.  

\paragraph{Correctness}
As we argue in the proof of Theorem \ref{thm:simple_alg}, it is enough to show that for all $\cE \supseteq X$ for which $\kappa(\cE) \le q \cdot \nfrac{R}{r}$:
\begin{align*}
    \cE_n \subseteq \sqrt{\magicnumber{\inparen{q \cdot \kappa(X)}}} \cdot \cE
\end{align*}
% \end{proof}

% \mybox{\begin{theorem}
% \label{thm:ellipsoid_algorithm_inclusion}
% Suppose that we give Algorithm \ref{alg:general_greedy_maxev} a value of $K$ satisfying $K = q\cdot\kappa(X)$. Let $E_q \coloneqq \inbraces{\cE \suchthat \kappa(\cE) \le q\cdot\kappa(X) \text{ and } X \subseteq \cE}$. Then, Algorithm \ref{alg:general_greedy_maxev} outputs an ellipsoid $\cE_n$ satisfying:
% \begin{align*}
%     \cE_n \subseteq \cE \cdot \sqrt{\magicnumber{\inparen{q\cdot\kappa(X)}}}, \text{ for all } \cE \in E_q
% \end{align*}
% \end{theorem}}
% \begin{proof}

\ynote{We should state it in a more direct way.} 

% \ynote{here is how we should start the proof of the main theorem.} 
% We should first prove the statement for one ellipsoid, defined by a matrix $J$ (say). Then write that we are going to define a potential $\Phi_t$ that can only go down throughout the execution of the algorithm (maybe we should be more precise).
% We will be able to bound $\Phi_n$ and then, using this upper bound, we will be able to derive an upper bound on the approximation ratio. We define $\Phi_t = (S_t - P_t)$. We now analyze how $S_t$ and $P_t$ change throughout the execution of the algorithm.
% nsm -- commented this out, because section 3 takes care of this bit now


Let $A_t \coloneqq U_t\Sigma_tV_t^T$, and observe that $\norm{A_tw} = \norm{\Sigma_t V_t^T w}$ for all $w\in\R^d$.

We assume without loss of generality that for all $t$, $\|A_{t-1}x_t\| > 1$, since Algorithm \ref{alg:general_greedy_maxev} ignores all points $x_t$ with $\|A_{t-1}x_t\| \leq 1$. In particular, when Algorithm \ref{alg:general_greedy_maxev} encounters such a point, it simply lets $A_t = A_{t-1}$.

For the purposes of our analysis, we will simulate the singular value correction step using the following procedure. If $w_{1,t}, \dots, w_{d,t}$ are the axes of our current ellipsoid at timestep $t$, then we will inject ``ghost'' points $x_{1,t}', \dots, x_{d,t}'$ such that $x_{i,t}'$ is in the same direction as $w_{i,t}'$ and $\norm{x_{i,t}'} = \sigma_{i,t}''$ as defined in Algorithm \ref{alg:general_greedy_maxev}. We can do this as per Lemma \ref{lemma:sv_update_step_simulation}.\ynote{the statement of the lemma and possibly its proof should appear here}

Observe that Lemma \ref{lemma:convenient_transformation} implies that it is sufficient to analyze $\sigma_{\max}\inparen{\astar \cdot A_{n}^{-1}}$ for our choice of $\astar$ whose aspect ratio is at most $K = q\cdot\nfrac{R}{r}$. Specifically, our goal is now to show that\\ $\sigma_{\max}\inparen{\astar \cdot A_{n}^{-1}}^2 \le \magicnumber{K}$.

We now prove the following lemmas.

\mybox{\begin{lemma}
\label{lemma:invariants}
Let $P_t \coloneqq 2\log\detv{\astar\cdot A_{t}^{-1}}$, $S_t \coloneqq \fnorm{\astar \cdot A_{t}^{-1}}^2$, and\\ $Q_t \coloneqq \max_{1\le i \le t} \norm{\astar x_i}^2$. 
Then, under the update rule for Algorithm \ref{alg:general_greedy_maxev}, we have:
\begin{align*}
    S_{t} - S_{t-1} &\le \min\inbraces{d,\inparen{P_{t} - P_{t-1}}} \cdot Q_t
\end{align*}
\end{lemma}}
\begin{proof}
We will show that:
\begin{align*}
    S_{t} - S_{t-1} &\le \inparen{P_{t} - P_{t-1}} \cdot Q_t \\
    S_{t} - S_{t-1} &\le d \cdot Q_t
\end{align*}
Recall Lemma \ref{lemma:invariant_basic_stronger}, which states that for all $t$, we have:
\begin{align*}
    \fnorm{\astar \cdot A_t^{-1}}^2 - \fnorm{\astar \cdot A_{t-1}^{-1}}^2 &\le \inparen{2\log\detv{\astar \cdot A_t^{-1}} - 2\log\detv{\astar \cdot A_{t-1}^{-1}}}\norm{\astar \cdot x_t}^2
\end{align*}
It is easy to see that this rearranges to:
\begin{align*}
    S_{t} - S_{t-1} \le \inparen{P_{t} - P_{t-1}} \cdot Q_t
\end{align*}
which is exactly the first inequality that we wanted, absent of the correction step. We also have:
\begin{align*}
    S_t - S_{t-1} = \inparen{1 - \frac{1}{\norm{A_{t-1}x_t}^2}}\norm{\astar x_t}^2 \le \inparen{1 - \frac{1}{\norm{A_{t-1}x_t}^2}}Q_t \le Q_t
\end{align*}

We now incorporate the singular value correction step. By Lemma \ref{lemma:sv_update_step_simulation}, the correction step can be simulated by adding points of norm at most $\norm{x_t}$ aligned with the axes that are too short. In other words, let $w_{1,t}, \dots, w_{t,d}$ be unit vectors in the directions of the axes of ellipsoid $\cE_t$. These vectors are exactly the singular vectors of $A_t$. The correction step now consists of injecting the points $w_{i,t}\cdot \nfrac{\norm{x_t}}{K}$.

First, we show that $\norm{\astar w_{i,t} \cdot \nfrac{\norm{x_t}}{K}} \le \max_{i \in [t]} \norm{\astar x_t} = \sqrt{Q_t}$. To see this, we have:
\begin{align*}
    \norm{\astar w_{i,t} \cdot \frac{\norm{x_t}}{K}} &= \frac{\norm{x_t}}{K} \cdot \norm{\astar w_{i,t}} \\
    &\le \norm{x_t} \cdot \frac{\sigma_{\max}\inparen{\astar}}{\nfrac{K}{q}} \cdot \frac{1}{q} \\
    &\le \sigma_{\min}\inparen{\astar} \cdot \norm{x_t} \cdot \frac{1}{q} \\
    &\le \norm{\astar x_t} \\
    &\le \max_{i \in [t]} \norm{\astar x_t}
\end{align*}
where we use $q \ge 1$. Now, the desired result will follow from summing the invariant obtained earlier over all the ghost points that we are adding. In particular, we have that $S_t-S_{t-1} \le (P_t-P_{t-1})\cdot Q_{t}$, and the invariant will still hold as all the intermediate terms will telescope out. On the other hand, from each update, we have $S_{t}-S_{t-1}\le Q_t$; there are at most $d$ correction steps, which yields the additional factor of $d$, as desired.
\end{proof}

Next, we show that for any algorithm satisfying the invariants implied by Lemma \ref{lemma:invariants}, we have that the total length of all the axes is not too large.

\mybox{\begin{lemma}
Run Algorithm \ref{alg:general_greedy_maxev} for $n$ steps. Let $\sigma_{i,j}$ denote the $i$th singular value of $\astar A_{j}^{-1}$. If we have $Q_t \le 1$ for all $t$, then we have:
\begin{align*}
    \sum_{i=1}^d \sigma_{i,n}^2 < \magicnumber{K}
\end{align*}
\end{lemma}}
\begin{proof}
We begin with Lemma \ref{lemma:sum_over_interval}.
\mybox{\begin{lemma}
\label{lemma:sum_over_interval}
For any timestamps $u, t$ such that $1 \le u < t \le n$, we have:
\begin{align*}
    S_{t} &\le S_u + \min\begin{dcases} d\sum_{j=u+1}^{t} Q_{j} \\ P_t \cdot Q_t + 4d\log K \cdot Q_{t} + d\logv{\frac{1}{Q_{u}}} \cdot Q_{t}\end{dcases}
\end{align*}
\end{lemma}}
\begin{proof}
We begin with the conclusion of Lemma \ref{lemma:invariants}:
\begin{align*}
    S_{t} - S_{t-1} &\le \inparen{P_{t} - P_{t-1}} \cdot Q_t \\
    S_{t-1} - S_{t-2} &\le \inparen{P_{t-1} - P_{t-2}} \cdot Q_{t-1} \\
    &\vdots \\
    S_{u+1} - S_u &\le \inparen{P_{u+1} - P_u} \cdot Q_{u+1}
\end{align*}
for some $u < t$. Since the $Q_i$s form a nondecreasing sequence, we have:
\begin{align*}
    S_{t} - S_u &\le \inparen{P_{t} - P_u} \cdot Q_t
\end{align*}
Thus, for any sequence $\inbraces{u, u+1, \dots, t-1, t}$, we have:
\begin{align*}
    S_{t} - S_{u} &\le P_{t} \cdot Q_{t} - P_{u} \cdot Q_{u+1} - \sum_{j=u+1}^{t-1} P_{j} \cdot \inparen{Q_{j+1} - Q_{j}} \\
    \implies S_{t} - P_{t} \cdot Q_{t} &\le S_{u} - P_{u} \cdot Q_{u+1} - \sum_{j=u+1}^{t-1} P_{j} \cdot \inparen{Q_{j+1} - Q_{j}}
\end{align*}
First, we will analyze the $- P_{u} \cdot Q_{u+1}$ term. From Lemma \ref{lemma:iterate_singular_value_lb}, we have $\sigma_{i,u}^2 \ge q^2 \cdot \nfrac{Q_u}{K^4} \ge \nfrac{Q_u}{K^4}$, and we can lower bound $P_u$:
\begin{align*}
    P_{u} &= \sum_{i=1}^d \logv{\sigma_{i,u}^2} \\
    &\ge d \cdot \logv{\frac{Q_{u}}{K^4}} \\
    &= d\log Q_{u} - 4d\log K
\end{align*}
This gives an upper bound for $- P_{u} \cdot Q_{u+1}$:
\begin{align*}
   -P_{u} \cdot Q_{u+1} &\le 4 Q_{u+1} \cdot d\log K - d \cdot Q_{u+1} \log Q_{u} \\
    &\le 4Q_{u+1}d\log K + d \cdot Q_{u+1} \logv{\frac{1}{Q_{u}}}
\end{align*}
Next, let's analyze the $-\sum_{j=u+1}^{t-1} P_{j} \cdot \inparen{Q_{j+1} - Q_{j}}$ term, for which we desire an upper bound. Using the previous expansion for any $P_{u}$, we have:
\begin{align*}
    -P_{j} &\le 4\log K - d \log Q_{j} \\
    \implies -P_{j} \cdot \inparen{Q_{j+1} - Q_{j}} &\le \inparen{4d\log K - d \log Q_{j}} \cdot \inparen{Q_{j+1} - Q_{j}} \\
    &= 4d\log K \cdot \inparen{Q_{j+1} - Q_{j}} - d\log Q_{j} \cdot \inparen{Q_{j+1} - Q_{j}}
\end{align*}
This means that:
\begin{align*}
    -\sum_{j=u+1}^{t-1} P_{j} \cdot \inparen{Q_{j+1} - Q_{j}} &\le \sum_{j=u+1}^{t-1} 4d\log K \cdot \inparen{Q_{j+1} - Q_{j}} - d\log Q_{j} \cdot \inparen{Q_{j+1} - Q_{j}} \\
    &= 4d\log K \cdot \sum_{j=u+1}^{t-1}\inparen{Q_{j+1} - Q_{j}} - d\sum_{j=u+1}^{t-1} \log Q_{j} \cdot \inparen{Q_{j+1} - Q_{j}}\\
    &= 4d\log K \cdot \inparen{Q_{t} - Q_{u+1}} - d\sum_{j=u+1}^{t-1} \log Q_{j} \cdot \inparen{Q_{j+1} - Q_{j}}
\end{align*}
where we use the fact that $Q_{t} \in [0,1]$ for all $t$. Thus, for all sequences $\inbraces{u, u+1, \dots, t-1, t}$, we have:
\begin{align*}
    S_{t} - P_{t} \cdot Q_{t} &\le S_{u} + 4Q_{u+1}d\log K + 4d\log K \cdot \inparen{Q_{t} - Q_{u+1}} + \\
    &\quad d \cdot Q_{u+1} \logv{\frac{1}{Q_{u}}} - d\sum_{j=u+1}^{t-1} \log Q_{j} \cdot \inparen{Q_{j+1} - Q_{j}}
\end{align*}
Let $t$ be the largest index in $[n]$ for which $Q_{t} < 1$. We now have:
\begin{align*}
    S_{t} - P_{t} \cdot Q_{t} &\le S_{u} + 4Q_{u+1}d\log K + 4d\log K \cdot \inparen{Q_{t} - Q_{u+1}} + \\
    &\quad d \cdot Q_{u+1} \logv{\frac{1}{Q_{u}}} + d\sum_{j=u+1}^{t-1} \logv{\frac{1}{Q_{j}}} \cdot \inparen{Q_{j+1} - Q_{j}} \\
    &= S_{u} + 4d\log K \cdot Q_{t} + d \cdot Q_{u+1} \logv{\frac{1}{Q_{u}}} + d\sum_{j=u+1}^{t-1} \logv{\frac{1}{Q_{j}}} \cdot \inparen{Q_{j+1} - Q_{j}} \\
    &\le S_{u} + 4d\log K \cdot Q_{t} + d \cdot Q_{u+1} \logv{\frac{1}{Q_{u}}} + d\logv{\frac{1}{Q_{u+1}}} \cdot \inparen{Q_{t} - Q_{u+1}} \\
    &\le S_{u} + 4d\log K \cdot Q_{t} + d \cdot Q_{u+1} \logv{\frac{1}{Q_{u}}} + d\logv{\frac{1}{Q_{u}}} \cdot \inparen{Q_{t} - Q_{u+1}} \\
    &= S_{u} + 4d\log K \cdot Q_{t} + d\logv{\frac{1}{Q_{u}}} \cdot Q_{t}
\end{align*}

Next, recall that we can also write, using the conclusion of Lemma \ref{lemma:invariants}:
\begin{align*}
    S_{t} - S_{u} &\le d\sum_{j=u+1}^{t} Q_{j}
\end{align*}
Combining, we have:
\begin{align*}
    S_{t} &\le S_u + \min\begin{dcases} d\sum_{j=u+1}^{t} Q_{j} \\ P_t \cdot Q_t + 4d\log K \cdot Q_{t} + d\logv{\frac{1}{Q_{u}}} \cdot Q_{t}\end{dcases}
\end{align*}
as desired.
\end{proof}

Observe that by Lemma \ref{lemma:sum_over_interval}, we have for any $1 \le u < t \le n$:
\begin{align*}
    S_{t} &\le S_u + \min\begin{dcases} d\sum_{j=u+1}^{t} Q_{j} \\ P_t \cdot Q_t + 4d\log K \cdot Q_{t} + d\logv{\frac{1}{Q_{u}}} \cdot Q_{t}\end{dcases}
\end{align*}

We now consider two cases.

\paragraph{Case 1: For all $t$, we have $Q_t > e^{-1}$.}
Let $u = 1$ and $t = n$. Then:
\begin{align*}
    S_n - P_n \cdot Q_n &\le 4d\log K \cdot Q_n + d \cdot Q_n \\
    &\le 4d\log K + d \\
    \implies \sum_{i=1}^d \sigma_{i,t}^2 - \logv{\sigma_{i,t}^2} &\le 4d\log K + d \\
    \implies \sum_{i=1}^d \sigma_{i,t}^2 &\le \frac{e}{e-1}\inparen{4d\log K + d}
\end{align*}
which is enough to conclude the proof in this case.

\paragraph{Case 2: There exists $t$ such that $Q_t \le e^{-1}$.}

Consider some subsequence of timestamps $t_0 > t_1 > \dots > t_m$ and notice that the above can be rewritten as:
\begin{align*}
    S_{t_i} &\le S_{t_{i+1}} + \min\begin{dcases}d\sum_{j=t_{i+1}+1}^{t_i} Q_{j} \\ P_{t_i}\cdot Q_{t_i}+4d\log K \cdot Q_{t_i} + d\logv{\frac{1}{Q_{t_{i+1}}}}\cdot Q_{t_i}\end{dcases} \\
    &= S_{t_{i+1}} + \min\begin{dcases}d\sum_{j=t_{i+1}+1}^{t_i} Q_{j} \\ P_{t_i}\cdot Q_{t_i}+4d\log K \cdot Q_{t_i} + d\logv{\frac{1}{Q_{t_{i}}}}\cdot Q_{t_i} + d\logv{\frac{Q_{t_i}}{Q_{t_{i+1}}}}\cdot Q_{t_i}\end{dcases}
\end{align*}

Now, use Fact \ref{fact:nice_sequence} to draw a nonincreasing sequence of indices $t_1, u_1, \dots, t_i, u_i, \dots, t_m$ such that:
\begin{itemize}
    \item For all $i \in [m]$, we have $Q_{t_i} \le e^{-i}$.
    \item For all $i \in [m]$, either $\nfrac{Q_{t_{i-1}}}{Q_{t_i}} \le e$ or: \begin{itemize}
        \item $\nfrac{Q_{t_{i-1}}}{Q_{u_{i-1}}} \le e$, and:
        \item $u_{i-1} = t_{i}+1$
    \end{itemize}
    \item For all $i \in [m]$, we either have $t_i = u_i$ or $\nfrac{Q_{t_i}}{Q_{u_i}} \le e$.
\end{itemize}
Our goal is to sum the above inequality over the sequence of indices $t_1, u_1, \dots, t_i, u_i, \dots, t_m$. To do so, we expand the above minimization into extra cases. In the first case, we have $\nfrac{Q_{t_i}}{Q_{t_{i+1}}} \le e$, from which we have:
\begin{align*}
    S_{t_i} &\le S_{t_{i+1}} + P_{t_i}\cdot e^{-i} + 4d\log K \cdot e^{-i} + d\cdot\frac{i}{e^i} + d\cdot e^{-i}
\end{align*}
In the second, we have $\nfrac{Q_{t_i}}{Q_{t_{i+1}}} > e$, which means $\nfrac{Q_{t_i}}{Q_{u_i}} \le e$ and $u_{i} = t_{i+1}+1$. Thus, we have:
\begin{align*}
    S_{u_i} &\le S_{t_{i+1}} + d\cdot Q_{u_i} \le S_{t_{i+1}} + d\cdot Q_{t_i} \le S_{t_{i+1}} + d\cdot e^{-i}
\end{align*}
And we have the following inequality to bridge $t_i$ to $u_i$:
\begin{align*}
    S_{t_i} &\le S_{u_i} + P_{t_i}\cdot Q_{t_i} + 4d\log K \cdot Q_{t_i} + d\logv{\frac{1}{Q_{t_{i}}}}\cdot Q_{t_i} + d\logv{\frac{Q_{t_i}}{Q_{u_i}}} \cdot Q_{t_i} \\
    &\le S_{u_i} + P_{t_i}\cdot e^{-i} + 4d\log K \cdot e^{-i} + d\cdot\frac{i}{e^i} + d\cdot e^{-i}
\end{align*}
% and the following to bridge $u_i$ to $t_{i+1}$ (it is easy to see via an argument similar to the above that $u_i = t_{i+1}+1$):
% \begin{align*}
%     S_{u_i} &\le S_{t_{i+1}} + d \cdot Q_{u_i} \le S_{t_{i+1}} + d\cdot e^{-i}
% \end{align*}
Adding the two gives:
\begin{align*}
    S_{t_i} &\le S_{t_{i+1}} + P_{t_i}\cdot e^{-i} + 4d\log K \cdot e^{-i} + d\cdot\frac{i}{e^i} + d\cdot e^{-i} + d\cdot e^{-i}
\end{align*}
Therefore, regardless of the value of $\nfrac{Q_{t_{i}}}{Q_{t_{i+1}}}$, we have:
\begin{align*}
    S_{t_i} &\le \max\begin{dcases} S_{t_{i+1}} + P_{t_i}\cdot e^{-i} + 4d\log K \cdot e^{-i} + d\cdot\frac{i}{e^i} + d\cdot e^{-i} \\ S_{t_{i+1}} + P_{t_i}\cdot e^{-i} + 4d\log K \cdot e^{-i} + d\cdot\frac{i}{e^i} + d\cdot e^{-i} + d\cdot e^{-i}\end{dcases} \\
    &\le S_{t_{i+1}} + P_{t_i}\cdot e^{-i} + 4d\log K \cdot e^{-i} + d\cdot\frac{i}{e^i} + d\cdot e^{-i} + d\cdot e^{-i} \\
    \implies S_{t_1} &\le S_{t_m} + \sum_{i=1}^{\infty} P_{t_i}\cdot e^{-i} + 4d\log K \sum_{i=1}^{\infty} e^{-i} + d\sum_{i=1}^{\infty}\frac{i}{e^i} + 2d\sum_{i=1}^{\infty} e^{-i} \\
    &\le S_{t_m} + \frac{P_{t_1}}{e-1} + \frac{4}{e-1}\cdot d\log K + d\cdot\frac{e}{(e-1)^2} + \frac{2d}{e-1}
\end{align*}
Finally, we use our original bound to write:
\begin{align*}
    S_{t_0} &\le S_{t_1} + P_{t_0} + 4d\log K \\
    &\le S_{t_m} + \frac{P_{t_1}}{e-1} + \frac{4}{e-1}\cdot d\log K + d\cdot\frac{e}{(e-1)^2} + \frac{2d}{e-1} + P_{t_0} + 4d\log K \\
    &\le S_{t_m} + P_{t_0}\cdot\frac{e}{e-1} + \frac{4}{e-1}\cdot d\log K + d\cdot\frac{e}{(e-1)^2} + \frac{2d}{e-1} + 4d\log K \\
    &\le d + P_{t_0}\cdot\frac{e}{e-1} + \frac{4}{e-1}\cdot d\log K + d\cdot\frac{e}{(e-1)^2} + \frac{2d}{e-1} + 4d\log K \\
    &< d + P_{t_0}\cdot\frac{e}{e-1} + 3d\log K + 3d + 4d\log K \\
    &= 7d\log K + P_{t_0}\cdot\frac{e}{e-1} + 4d \\
    \implies 4d + 7d\log K &> \sum_{i=1}^d \sigma_{i,n}^2 - \frac{e}{e-1}\logv{\sigma_{i,n}^2} \\
    &\ge \frac{e-2}{e-1}\sum_{i=1}^d \sigma_{i,n}^2 \\
    \implies \sum_{i=1}^d \sigma_{i,n}^2 &< 7d\log K \cdot \frac{e-1}{e-2} + 4d \cdot \frac{e-1}{e-2} < \magicnumber{K}
\end{align*}
as desired.
\end{proof}
Notice that the rest of the proof follows from the following statement:
\begin{align*}
    \sigmamax{n}^2 < \sum_{i=1}^d \sigma_{i,n}^2 < \magicnumber{K}
\end{align*}
which is exactly what we wanted.
\end{proof}

==> main_optimal_updates.tex <==
\section{Characterizing Optimal Update Rules}
\label{section:optimal_updates}

The below holds for all monotonic algorithms for Problem \ref{problem:main_problem}.

\textcolor{red}{This is a heavily abbreviated argument; if we keep it, this will have to be rewritten significantly.}

\mybox{\begin{lemma}
Let $z \coloneqq A_{t-1}x_t$.

If $A_t = \widehat{A}A_{t-1}$ for some symmetric matrix $\widehat{A}$ with eigenvalues $\lambda_1^{-1},\dots,\lambda_d^{-1}$ and unit eigenvectors $v_1,\dots,v_d$, then every update rule satisfies the following invariants:
\begin{align*}
    \frac{S_{t}-S_{t-1}}{P_{t}-P_{t-1}} &= \frac{\sum_{i=1}^d\inparen{\lambda_i^2-1}\norm{A_{t-1}^{-1}v_i}^2}{\sum_{i=1}^d \logv{\lambda_i^2}}
\end{align*}
where:
\begin{align*}
    \lambda_i &\ge 1 & \sum_{i=1}^d \frac{1}{\lambda_i^2}\ip{v_i, z}^2 &\le 1
\end{align*}
\end{lemma}}
\begin{proof}[Proof outline]
Follow the same calculation steps as done in the original invariants analysis.
\end{proof}

We use this to obtain a lower bound on the evolution of our potential functions for every monotonic algorithm:

\mybox{\begin{lemma}
We have:
\begin{align*}
    \frac{S_{t}-S_{t-1}}{P_{t}-P_{t-1}} &\ge \sigma_{\min}\inparen{A_{t-1}^{-1}}^2
\end{align*}
\end{lemma}}
\begin{proof}
From the monotonicity constraint, it is easy to see that we must have $\lambda_i \ge 1$ for all $i \in [d]$. Next, given that the ellipsoid determined by $\widehat{A}$ must cover $z$, we have that there exists at least one $i$ such that $\lambda_i \ge \norm{z}$. For this value of $i$, we must be able to write:
\begin{align*}
    \frac{S_{t}-S_{t-1}}{P_{t}-P_{t-1}} = \frac{\sum_{i=1}^d\inparen{\lambda_i^2-1}\norm{A_{t-1}^{-1}v_i}^2}{\sum_{i=1}^d \logv{\lambda_i^2}} \ge \frac{\norm{z}^2 - 1}{2\log\norm{z}} \cdot \norm{A_{t-1}^{-1}v_i}^2 \ge \sigma_{\min}\inparen{A_{t-1}^{-1}}^2
\end{align*}
\end{proof}

Now, consider the following family of instances. We initialize $\cE_0 = \inbraces{x \suchthat \norm{x} \le 1}$. Next, we initialize the convex body $X$ to be a sufficiently discretized version of the ellipsoid:
\begin{align*}
\cE = \inbraces{x \suchthat \sum_{i=1}^d \frac{x_i^2}{\inparen{\sigma_d \cdot \nfrac{\sigma_i}{\sigma_1^2}}^2} \le 1}\text{ where }\sigma_1 \le \dots \le \sigma_d
\end{align*}
Loosely speaking, we will give points on some sufficiently discretized form of the ``great circle'' connecting $\sigma_d \cdot \nfrac{\sigma_i}{\sigma_1^2} \cdot e_i$ to $\sigma_d \cdot \nfrac{\sigma_{i+1}}{\sigma_1^2} \cdot e_{i+1}$, for all $i \in [d-1]$.

